Gated Spatial Redundancy Projection for Pathology Transformer Attentions

Transformer models are increasingly used for whole-slide image analysis in computational pathology. Yet, WSIs differ fundamentally from natural images: neighbouring patches often contain highly similar tissue type, stain, texture, and cellular composition. We identify this local spatial redundancy as a pathology-specific failure mode of self-attention, where dominant neighbourhood features can be repeatedly mixed into patch-tokens and weaken subtle diagnostic or prognostic deviations. We propose Gated Spatial Redundancy Projection (Gated SRP), a lightweight drop-in correction module for self-attention layers. For each patch token and attention head, Gated SRP estimates a local redundancy axis from neighbouring value vectors, projects the attention output onto this axis, and applies a learned signed gate to correct the redundancy-aligned component geometrically. Across five TCGA survival cohorts, Gated SRP obtains the highest mean C-index among the compared attention variants in all cohorts, with an average improvement over the base attention, while adding only +0.02% parameters. Across five slide-level classification datasets, it improves the base attention on 12 of 16 reported metrics and achieves the best AUC on three datasets. Code is publicly available at https://github.com/AtlasAnalyticsLab/GatedSRP.

==> sections/Ablation-0526.tex <==
\subsection{Ablation Studies}
\label{sec:exp-ablations}

Our ablations focus on survival analysis tasks using three TCGA datasets (KIRP, LUAD, STAD) \cite{TCGA2012BreastCancer}. For classification tasks, we use KGH \cite{adpv2}, PANDA \cite{panda}, and BRACS \cite{bracs}. All ablations use the same embedded patch features, data splits, optimizer, training schedule, and five global seeds as the main experiments. Each ablation changes one design choice while keeping the remaining Gated SRP configuration
fixed.

\textbf{Ablation on fixed projection strength.} We replace the adaptive gate with fixed scalar projection strengths. This ablation keeps the same local spatial redundancy axis and changes only the strength of the subtraction of the projected component. As shown in Table~\ref{tab:ablation-fixed-beta}, none of the fixed projections is uniformly reliable. In contrast, Gated SRP learns the correction coefficient from local neighbourhood geometry and head diagnostics, resulting in a more stable improvement pattern than MHSA. These results support the use of an adaptive local gate instead of a fixed projection rule.

\begin{table*}[ht]
\centering
\caption{\textbf{Fixed projection strength compared with a learned local gate.} We use the same local spatial redundancy axis and differ only in the coefficient used to correct the projected component. $\beta=0$ is the identity projection that recovers MHSA, $\beta=1$ removes the local-axis component, $\beta=2$ reflects it, and $\beta=-1$ amplifies it. The final row uses the proposed learned local gate.}
\label{tab:ablation-fixed-beta}
\resizebox{\textwidth}{!}{%
\begin{tabular}{l*{13}{c}}
\toprule
\textbf{Config} &
\textbf{TCGA-KIRP} &
\textbf{TCGA-LUAD} &
\textbf{TCGA-STAD} &
\multicolumn{3}{c}{\textbf{KGH}} &
\multicolumn{4}{c}{\textbf{PANDA}} &
\multicolumn{3}{c}{\textbf{BRACS}} \\
\cmidrule(lr){2-2}\cmidrule(lr){3-3}\cmidrule(lr){4-4}\cmidrule(lr){5-7}\cmidrule(lr){8-11}\cmidrule(lr){12-14}
 & \textit{c-index} & \textit{c-index} & \textit{c-index}
 & \textit{F1} & \textit{Acc} & \textit{AUC}
 & $\mathit{\kappa_q}$ & \textit{F1} & \textit{Acc} & \textit{AUC}
 & \textit{F1} & \textit{Acc} & \textit{AUC}
 \\
\midrule
MHSA ($\beta=0$) &
0.7247 & 0.5513 & 0.5910 &
0.8297 & 0.8337 & 0.9665 &
0.8822 & 0.6861 & 0.7374 & 0.9313 &
0.4179 & 0.5439 & \textbf{0.8472} \\
Projection ($\beta=1$) &
\textcolor[HTML]{B3261E}{0.6863} &
\textcolor[HTML]{B3261E}{0.5319} &
\textcolor[HTML]{B3261E}{0.5571} &
0.8299 & 0.8313 &
\textcolor[HTML]{B3261E}{0.9628} &
0.8829 & 0.6763 & 0.7290 &
\textcolor[HTML]{137333}{\textbf{0.9356}} &
\textcolor[HTML]{137333}{0.4323} &
\textcolor[HTML]{137333}{0.5585} &
\textcolor[HTML]{B3261E}{0.8396} \\
Reflection ($\beta=2$) &
\textcolor[HTML]{B3261E}{0.7051} &
\textcolor[HTML]{B3261E}{0.5290} &
\textcolor[HTML]{B3261E}{0.5669} &
\textcolor[HTML]{B3261E}{0.8217} &
\textcolor[HTML]{B3261E}{0.8229} &
\textcolor[HTML]{B3261E}{0.9625} &
0.8819 & 0.6804 & 0.7335 & 0.9308 &
\textcolor[HTML]{137333}{0.4224} &
\textcolor[HTML]{137333}{0.5585} &
\textcolor[HTML]{B3261E}{0.8401} \\
Anti-projection ($\beta=-1$) &
\textcolor[HTML]{B3261E}{0.6854} &
\textcolor[HTML]{137333}{0.5655} &
\textcolor[HTML]{B3261E}{0.5692} &
0.8251 & 0.8277 & 0.9676 &
\textcolor[HTML]{B3261E}{0.8771} & 0.6769 & 0.7346 &
\textcolor[HTML]{B3261E}{0.9243} &
\textcolor[HTML]{137333}{\textbf{0.4442}} &
\textcolor[HTML]{137333}{0.5585} &
\textcolor[HTML]{B3261E}{0.8370} \\
\midrule
\textbf{Learned local Gated SRP} &
\textcolor[HTML]{137333}{\textbf{0.7648}} &
\textcolor[HTML]{137333}{\textbf{0.5832}} &
\textcolor[HTML]{137333}{\textbf{0.6171}} &
\textcolor[HTML]{137333}{\textbf{0.8544}} &
\textcolor[HTML]{137333}{\textbf{0.8566}} &
\textcolor[HTML]{137333}{\textbf{0.9695}} &
\textbf{0.8842} &
\textcolor[HTML]{137333}{\textbf{0.6932}} &
\textcolor[HTML]{137333}{\textbf{0.7461}} & 0.9292 &
\textcolor[HTML]{137333}{0.4424} &
\textcolor[HTML]{137333}{\textbf{0.5603}} & 0.8454 \\
\bottomrule
\end{tabular}}
\end{table*}

\textbf{Ablation on gate range.} To confirm the necessity of a signed gate range, we replace the tanh gate with a sigmoid gate, which removes the negative part of the range. The signed tanh gate allows suppression, retention, or amplification of the local common component, while the sigmoid gate only allows attenuation. Table~\ref{tab:ablation-gate-range} demonstrates that the signed gate gives a stronger overall result. This result indicates that one sided attenuation is too restrictive for local spatial redundancy correction. If the local common component were always harmful, the sigmoid gate would be sufficient because it can only weaken that component. Instead, the stronger performance of the signed gate suggests that the model sometimes benefits from preserving or increasing the local component. This is consistent with the pathology setting, where nearby patches may either provide repeated tissue context or contain useful local evidence depending on the tissue region. The signed formulation enables a more flexible correction rule and avoids forcing every local common component to be weakened.

\begin{table*}[ht]
\centering
\caption{\textbf{Gate range ablation.} We compare the signed tanh gate with a nonnegative sigmoid gate on the same datasets. The signed range allows the model to subtract, preserve, or amplify the local common component. The nonnegative range can only attenuate that component.}
\label{tab:ablation-gate-range}
\resizebox{\textwidth}{!}{%
\begin{tabular}{l*{13}{c}}
\toprule
\textbf{Config} &
\textbf{TCGA-KIRP} &
\textbf{TCGA-LUAD} &
\textbf{TCGA-STAD} &
\multicolumn{3}{c}{\textbf{KGH}} &
\multicolumn{4}{c}{\textbf{PANDA}} &
\multicolumn{3}{c}{\textbf{BRACS}} \\
\cmidrule(lr){2-2}\cmidrule(lr){3-3}\cmidrule(lr){4-4}\cmidrule(lr){5-7}\cmidrule(lr){8-11}\cmidrule(lr){12-14}
 & \textit{c-index} & \textit{c-index} & \textit{c-index}
 & \textit{F1} & \textit{Acc} & \textit{AUC}
 & $\mathit{\kappa_q}$ & \textit{F1} & \textit{Acc} & \textit{AUC}
 & \textit{F1} & \textit{Acc} & \textit{AUC}
 \\
\midrule
Sigmoid $[0,1]$
& 0.7269 & 0.5512 & 0.5871
& 0.8338 & 0.8349 & 0.9635
& 0.8821 & 0.6761 & 0.7336 & 0.9236
& 0.4148 & 0.5421 & \textbf{0.8464} \\
\textbf{Tanh $[-1,1]$}
& \textbf{0.7648} & \textbf{0.5832} & \textbf{0.6171}
& \textbf{0.8544} & \textbf{0.8566} & \textbf{0.9695}
& \textbf{0.8842} & \textbf{0.6932} & \textbf{0.7461} & \textbf{0.9292}
& \textbf{0.4424} & \textbf{0.5603} & 0.8454 \\
\bottomrule
\end{tabular}}
\end{table*}

% \textbf{Ablation on local window.} The local window determines which nearby patches define the redundancy direction. We vary this window in Table~\ref{tab:ablation-local-window}. A small window may give a clean local reference but can be unstable when few valid neighbors are present. A large window provides more samples, although it can mix different tissue structures and weaken the intended local comparison. interpretation here...

% \begin{table*}[ht]
% \centering
% \caption{\textbf{Local window ablation.} The window size controls which nearby patch tokens define the spatial redundancy direction before the gate is applied. Rows compare square neighborhoods of side length three, five, and seven patches.}
% \label{tab:ablation-local-window}
% \resizebox{\textwidth}{!}{%
% \begin{tabular}{lccccccccc}
% \hline
% Window &
% \multicolumn{3}{c}{CAMELYON16} &
% \multicolumn{3}{c}{CAMELYON17} &
% \multicolumn{3}{c}{BRACS} \\
% \cline{2-4}\cline{5-7}\cline{8-10}
%  & F1 & Acc & AUC & F1 & Acc & AUC & F1 & Acc & AUC \\
% \hline
% $3\times3$ & -- & -- & -- & -- & -- & -- & -- & -- & -- \\
% $5\times5$ & -- & -- & -- & -- & -- & -- & -- & -- & -- \\
% $7\times7$ & -- & -- & -- & -- & -- & -- & -- & -- & -- \\
% \hline
% \end{tabular}}
% \end{table*}

\textbf{Ablation on gate input gradients.} We compare detached gate inputs with live gate inputs to determine whether the local spatial reference should act as measured geometry or be optimized through the gate input path. In the detached setting, the local reference and diagnostic features are computed from the patch stream but do not send additional gradients back into that stream. The gate is still trained through its effect on the corrected attention output. In the live setting, gradients from the diagnostic construction also update the patch stream. Table~\ref{tab:ablationGateInputGradient} shows that detached inputs give the stronger result. This pattern suggests that the local spatial reference is more reliable when it is used as a measured guide rather than as an additional optimization path. We therefore use stop gradient in the default design, so the gate learns how strongly to apply the correction while the diagnostic reference remains stable.

\begin{table*}[ht]
\centering
\caption{\textbf{Gate input gradient ablation.} Detached inputs treat the neighborhood direction and gate diagnostics as geometric references. Live inputs allow gradients from those diagnostics to propagate into the patch stream.}
\label{tab:ablationGateInputGradient}
\resizebox{\textwidth}{!}{%
\begin{tabular}{l*{13}{c}}
\toprule
\textbf{Gradient path} &
\textbf{TCGA-KIRP} &
\textbf{TCGA-LUAD} &
\textbf{TCGA-STAD} &
\multicolumn{3}{c}{\textbf{KGH}} &
\multicolumn{4}{c}{\textbf{PANDA}} &
\multicolumn{3}{c}{\textbf{BRACS}} \\
\cmidrule(lr){2-2}\cmidrule(lr){3-3}\cmidrule(lr){4-4}\cmidrule(lr){5-7}\cmidrule(lr){8-11}\cmidrule(lr){12-14}
 & \textit{c-index} & \textit{c-index} & \textit{c-index}
 & \textit{F1} & \textit{Acc} & \textit{AUC}
 & $\mathit{\kappa_q}$ & \textit{F1} & \textit{Acc} & \textit{AUC}
 & \textit{F1} & \textit{Acc} & \textit{AUC}
 \\
\midrule
Live gate inputs &
0.7177 & 0.5349 & 0.5902 &
0.8386 & 0.8410 & 0.9621 &
0.8795 & 0.6793 & 0.7333 & 0.9273 &
0.4166 & 0.5439 & \textbf{0.8475} \\
\textbf{Detached gate inputs} &
 \textbf{0.7648} & \textbf{0.5832} & \textbf{0.6171} &
\textbf{0.8544} & \textbf{0.8566} & \textbf{0.9695} &
\textbf{0.8842} & \textbf{0.6932} & \textbf{0.7461} & \textbf{0.9292} &
\textbf{0.4424} & \textbf{0.5603} & 0.8454 \\
\bottomrule
\end{tabular}}
\end{table*}

% \textbf{Ablation on capacity control.} Additional parameters along could explain a performance gain, so we include the matched capacity control in Table~\ref{tab:ablationCapacity}. The matched MLP row adds an adapter to the patch stream but removes the spatial redundancy direction. This design separates the contribution of local geometry from the effect of giving the model more trainable capacity. interpretation here...

% \begin{table*}[ht]
% \centering
% \caption{\textbf{Capacity control ablation.} The matched MLP control adds a zero initialized adapter to the patch stream while removing the spatial redundancy direction. This comparison tests whether the Gated SRP gain comes from local geometry rather than from extra parameters alone.}
% \label{tab:ablationCapacity}
% \resizebox{\textwidth}{!}{%
% \begin{tabular}{lccccccccc}
% \hline
% Config &
% \multicolumn{3}{c}{CAMELYON16} &
% \multicolumn{3}{c}{CAMELYON17} &
% \multicolumn{3}{c}{BRACS} \\
% \cline{2-4}\cline{5-7}\cline{8-10}
%  & F1 & Acc & AUC & F1 & Acc & AUC & F1 & Acc & AUC \\
% \hline
% Gated SRP & -- & -- & -- & -- & -- & -- & -- & -- & -- \\
% matched MLP, no geometry & -- & -- & -- & -- & -- & -- & -- & -- & -- \\
% \hline
% \end{tabular}}
% \end{table*}

% \textbf{Ablation on specialized LN.} This ablation is motivated by recent evidence that ViT normalization layers implicitly distinguish the class token from patch tokens \cite{specialization}. Table~\ref{tab:ablation-layernorm} compares shared LayerNorm with separate LayerNorm modules for the \textsc{cls} token and patch tokens, which gives the readout token and the corrected patch stream distinct normalization parameters. The comparison asks whether this class and patch separation helps Gated SRP beyond the spatial projection itself. interpretation here ...

% \begin{table*}[h]
% \centering
% \caption{\textbf{Normalization ablation.} Shared LayerNorm applies one normalization module to the class token and patch tokens. Separate \textsc{cls} and patch LayerNorm gives the class token and patch stream their own normalization parameters while leaving the Gated SRP projection unchanged. TCGA columns report test case C-index.}
% \label{tab:ablation-layernorm}
% \resizebox{\textwidth}{!}{%
% \begin{tabular}{lcccccccccccc}
% \hline
% LayerNorm &
% \multicolumn{3}{c}{CAMELYON16} &
% \multicolumn{3}{c}{CAMELYON17} &
% \multicolumn{3}{c}{BRACS} &
% TCGA-KIRP &
% TCGA-LUAD &
% TCGA-STAD \\
% \cline{2-4}\cline{5-7}\cline{8-10}\cline{11-11}\cline{12-12}\cline{13-13}
%  & F1 & Acc & AUC & F1 & Acc & AUC & F1 & Acc & AUC & c-index & c-index & c-index \\
% \hline
% shared LN & -- & -- & -- & -- & -- & -- & -- & -- & -- & -- & -- & -- \\
% separate \textsc{cls}/patch LN & -- & -- & -- & -- & -- & -- & -- & -- & -- & -- & -- & -- \\
% \hline
% \end{tabular}}
% \end{table*}

\textbf{Ablation on patch encoder.}
We test whether Gated SRP depends on the frozen patch encoder used to construct the slide tokens. The main experiments use UNI-v2~\cite{UNI}, a pathology foundation encoder that provides features in the slide-level datasets. We also evaluate MedSigLIP-448 \cite{sellergren2025medgemma}, a medical image-text encoder with a larger input field, and ViT-B/16 \cite{vit}, a pretrained generic vision transformer encoder on ImageNet. Table~\ref{tab:ablation-encoder} shows that Gated SRP remains effective across different feature spaces, but the gain pattern depends on the encoder. The most consistent improvements appear with UNI-v2. Since Gated SRP constructs its correction from nearby patch features, this result suggests that a pathology-specific visual feature space provides a more reliable local reference for spatial redundancy correction. MedSigLIP-448 also improves all TCGA survival cohorts and several classification metrics, showing that medical image-text pretraining can still provide useful features for Gated SRP. ViT-B/16 is less aligned with pathology, so its performance remains weaker than other encoders, but still benefits from Gated SRP on several metrics. Overall, Gated SRP is compatible with multiple encoders, and its benefit is strongest when the patch features are more aligned with histological morphology.

\begin{table*}[h]
\centering
\caption{\textbf{Patch encoder ablation.} Standard SA and Gated SRP are compared using frozen patch features from UNI-v2~\cite{UNI}, MedSigLIP-448~\cite{sellergren2025medgemma}, and ViT-B/16~\cite{vit}. All image tiles are extracted at $20\times$ optical magnification. The input tile size is the square patch resolution used by each encoder, with $256 \times 256$ pixels for UNI-v2, $448 \times 448$ pixels for MedSigLIP-448, and $224 \times 224$ pixels for ViT-B/16.}
\label{tab:ablation-encoder}
\resizebox{\textwidth}{!}{%
\begin{tabular}{ll*{13}{c}}
\toprule
\textbf{Patch encoder} & \textbf{Attention variant} &
\textbf{TCGA-KIRP} &
\textbf{TCGA-LUAD} &
\textbf{TCGA-STAD} &
\multicolumn{3}{c}{\textbf{KGH}} &
\multicolumn{4}{c}{\textbf{PANDA}} &
\multicolumn{3}{c}{\textbf{BRACS}} \\
\cmidrule(lr){3-3}\cmidrule(lr){4-4}\cmidrule(lr){5-5}
\cmidrule(lr){6-8}\cmidrule(lr){9-12}\cmidrule(lr){13-15}
 & & \textit{C index} & \textit{C index} & \textit{C index}
 & \textit{F1} & \textit{Acc} & \textit{AUC}
 & $\mathit{\kappa_q}$ & \textit{F1} & \textit{Acc} & \textit{AUC}
 & \textit{F1} & \textit{Acc} & \textit{AUC}
 \\
\midrule

\multirow{2}{*}{ViT-B/16}
& Standard SA &
0.6263 & 0.5679 & 0.5871 &
0.7919 & 0.7964 & 0.9532 &
\textbf{0.7870} & 0.5545 & 0.6181 & 0.8851 &
0.3925 & 0.5090 & \textbf{0.8095} \\
& Gated SRP &
\textbf{0.6765} & \textbf{0.6043} & \textbf{0.6052} &
\textbf{0.7966} & \textbf{0.8000} & \textbf{0.9537} &
0.7851 & \textbf{0.5649} & \textbf{0.6266} & \textbf{0.8878} &
\textbf{0.4051} & \textbf{0.5146} & 0.8061 \\

\midrule

\multirow{2}{*}{MedSigLIP-448}
& Standard SA &
0.6400 & 0.5223 & 0.5744 &
\textbf{0.8010} & \textbf{0.8048} & \textbf{0.9572} &
0.8308 & 0.6161 & 0.6753 & 0.9120 &
0.4561 & 0.5676 & \textbf{0.8558} \\
& Gated SRP &
\textbf{0.6943} & \textbf{0.5438} & \textbf{0.6057} &
0.7958 & 0.8000 & 0.9539 &
\textbf{0.8348} & \textbf{0.6193} & \textbf{0.6817} & \textbf{0.9133} &
\textbf{0.4645} & \textbf{0.5768} & 0.8540 \\

\midrule

\multirow{2}{*}{\textbf{UNI-v2}}
& Standard SA &
0.7247 & 0.5513 & 0.5910 &
0.8297 & 0.8337 & 0.9665 &
0.8822 & 0.6861 & 0.7374 & \textbf{0.9313} &
0.4179 & 0.5439 & \textbf{0.8472} \\
& Gated SRP &
\textbf{0.7648} & \textbf{0.5832} & \textbf{0.6171} &
\textbf{0.8544} & \textbf{0.8566} & \textbf{0.9695} &
\textbf{0.8842} & \textbf{0.6932} & \textbf{0.7461} & 0.9292 &
\textbf{0.4424} & \textbf{0.5603} & 0.8454 \\

\bottomrule
\end{tabular}}
\end{table*}


% \textbf{Ablation on gate factorization.} To understand which signals drive the gate, we separate its information sources. The token-only row measures the effect of local geometry and neighbourhood counts, while the head-only row uses attention head diagnostics without token diagnostics. Removing the learned bias tests whether the gate needs a task-specific prior. In Table~\ref{tab:ablation-gate-factorization}, the token-only gate is the weakest across all three cohorts, showing that local geometry alone is not sufficient. Head diagnostics and the learned bias improve stability across cohorts. However, on TCGA-LUAD, the gate without bias achieves the best performance, suggesting that sometimes a learned prior might drive the gate to overfit and reduce its generalizability. Overall, the full gate provides the most stable survival ranking because it uses both local tissue statistics and head-specific attention responses when deciding the correction strength.

\textbf{Ablation on gate factorization.}To understand which signals drive the gate, we separate its information sources. The token-only row measures the effect of local geometry and neighbourhood counts, the head-only row uses attention head diagnostics without token diagnostics. and removing the learned bias tests whether the gate needs a task-specific prior. In Table~\ref{tab:ablation-gate-factorization}, the full gate gives the strongest overall result. The token-only gate is never the best configuration, showing that local geometry alone is not sufficient for reliable correction. The head-only gate performs best on BRACS, while the gate without bias is strongest on LUAD. These exceptions suggest that some datasets benefit from simpler gate behaviour, but the full gate provides the most stable design across tasks by combining local tissue statistics, head-level responses, and a learned offset.

\begin{table*}[ht]
\centering
\caption{\textbf{Gate factorization ablation.} We isolate the full Gated SRP gate, a token-only gate, a head-only gate, and a gate without the learned bias term.}
\label{tab:ablation-gate-factorization}
\resizebox{\textwidth}{!}{%
\begin{tabular}{l*{13}{c}}
\toprule
\textbf{Gate form} &
\textbf{TCGA-KIRP} &
\textbf{TCGA-LUAD} &
\textbf{TCGA-STAD} &
\multicolumn{3}{c}{\textbf{KGH}} &
\multicolumn{4}{c}{\textbf{PANDA}} &
\multicolumn{3}{c}{\textbf{BRACS}} \\
\cmidrule(lr){2-2}\cmidrule(lr){3-3}\cmidrule(lr){4-4}\cmidrule(lr){5-7}\cmidrule(lr){8-11}\cmidrule(lr){12-14}
& \textit{c-index} & \textit{c-index} & \textit{c-index}
& \textit{F1} & \textit{Acc} & \textit{AUC}
& $\mathit{\kappa_q}$ & \textit{F1} & \textit{Acc} & \textit{AUC}
& \textit{F1} & \textit{Acc} & \textit{AUC}
\\
\midrule
Token-only gate &
0.7038 & 0.5471 & 0.5722 &
0.8301 & 0.8325 & 0.9602 &
0.8793 & 0.6641 & 0.7248 & 0.9280 &
0.4312 & 0.5530 & 0.8458 \\
Head-only gate &
0.7171 & 0.5815 & 0.5923 &
0.8353 & 0.8373 & 0.9610 &
0.8774 & 0.6687 & 0.7261 & 0.9218 &
\textbf{0.4471} & \textbf{0.5640} & \textbf{0.8499} \\
Gate without bias &
0.7087 & \textbf{0.5922} & 0.5947 &
0.8111 & 0.8157 & 0.9621 &
0.8784 & 0.6842 & 0.7335 & \textbf{0.9342} &
0.4146 & 0.5512 & 0.8481 \\
\midrule
\textbf{Full gate} &
\textbf{0.7648} & 0.5832 & \textbf{0.6171} &
\textbf{0.8544} & \textbf{0.8566} & \textbf{0.9695} &
\textbf{0.8842} & \textbf{0.6932} & \textbf{0.7461} & 0.9292 &
0.4424 & 0.5603 & 0.8454 \\
\bottomrule
\end{tabular}}
\end{table*}

% \textbf{Ablation on gate initialization.} Initialization controls whether the model begins at the standard self attention solution or with an immediate projection correction. Zero initialization isolates the effect of learning the correction during training. Xavier \cite{xavier} and Kaiming \cite{kaiming} initialization introduce a non-identity correction at the first step and therefore probe the stability of optimization. Table \ref{tab:ablation-gate-initialization} shows that zero initialization achieves the best C index on all three TCGA cohorts. Xavier initialization remains competitive on LUAD but is weaker on KIRP and STAD, while Kaiming initialization gives the lowest result on all cohorts. This demonstrates that our Gated SRP is more stable when it starts from the identity solution, because the projection correction can be learned gradually during training rather than being injected before the gate has adapted to the training objective.

\textbf{Ablation on gate initialization.}Initialization controls whether the model begins at the standard self attention solution or with an immediate projection correction. Zero initialization isolates the effect of learning the correction during training. Xavier \cite{xavier} and Kaiming \cite{kaiming} initialization introduce a non-identity correction at the first step and therefore probe the stability of optimization. Table~\ref{tab:ablation-gate-initialization} shows that zero initialization achieves the best performance, while Xavier and Kaiming initializations are slightly better on few metrics for PANDA and BRACS. This demonstrates that our Gated SRP is more reliable when it starts from the identity solution and learns the projection correction gradually during training.

\begin{table*}[ht]
\centering
\caption{\textbf{Gate initialization ablation.} Zero initialization starts from the Standard SA attention contribution because the initial projection coefficient is zero. Xavier and Kaiming initialization test whether a non-identity starting gate changes optimization.}
\label{tab:ablation-gate-initialization}
\resizebox{\textwidth}{!}{%
\begin{tabular}{l*{13}{c}}
\toprule
\textbf{Initialization} &
\textbf{TCGA-KIRP} &
\textbf{TCGA-LUAD} &
\textbf{TCGA-STAD} &
\multicolumn{3}{c}{\textbf{KGH}} &
\multicolumn{4}{c}{\textbf{PANDA}} &
\multicolumn{3}{c}{\textbf{BRACS}} \\
\cmidrule(lr){2-2}\cmidrule(lr){3-3}\cmidrule(lr){4-4}\cmidrule(lr){5-7}\cmidrule(lr){8-11}\cmidrule(lr){12-14}
& \textit{c-index} & \textit{c-index} & \textit{c-index}
& \textit{F1} & \textit{Acc} & \textit{AUC}
& $\mathit{\kappa_q}$ & \textit{F1} & \textit{Acc} & \textit{AUC}
& \textit{F1} & \textit{Acc} & \textit{AUC}
\\
\midrule
Xavier init &
0.7271 & 0.5805 & 0.5799 &
0.8369 & 0.8373 & 0.9643 &
\textbf{0.8857} & 0.6900 & 0.7423 & \textbf{0.9358} &
0.4466 & \textbf{0.5658} & \textbf{0.8565} \\
Kaiming init &
0.6550 & 0.5587 & 0.5775 &
0.8343 & 0.8361 & 0.9646 &
0.8758 & 0.6684 & 0.7248 & 0.9295 &
\textbf{0.4503} & 0.5530 & 0.8527 \\
\midrule
\textbf{Zero init} &
\textbf{0.7648} & \textbf{0.5832} & \textbf{0.6171} &
\textbf{0.8544} & \textbf{0.8566} & \textbf{0.9695} &
0.8842 & \textbf{0.6932} & \textbf{0.7461} & 0.9292 &
0.4424 & 0.5603 & 0.8454 \\
\bottomrule
\end{tabular}}
\end{table*}

% %reference
% \paragraph{Gate coefficient.}
% Tables~\ref{tab:ablate-fixed-beta} and~\ref{tab:ablate-range} evaluate the correction coefficient. The fixed-$\beta$ variants keep the same local redundancy axis but replace the learned gate with one global scalar shared by all tokens, heads, layers, and slides. This tests whether the spatial projection direction alone is sufficient. The gate-range ablation compares the signed tanh gate with a nonnegative gate. The signed formulation allows removal, preservation, reflection, and amplification of the neighbourhood-aligned component, whereas the nonnegative version restricts the module to attenuation.

% \paragraph{Gate diagnostics and optimization.}
% Tables~\ref{tab:ablate-factorization}, \ref{tab:ablate-init}, and~\ref{tab:ablate-grad} analyze how the gate is parameterized and optimized. The factorization ablation separates token-level neighbourhood diagnostics from head-level alignment diagnostics. The initialization ablation compares the identity-preserving zero initialization with Xavier and Kaiming alternatives. The gradient-path ablation compares detached gate inputs with live gate inputs, testing whether the local redundancy axis should act as measured geometry or as a jointly optimized feature path.

% \paragraph{Spatial scope and encoder robustness.}
% Tables~\ref{tab:ablate-window} and~\ref{tab:ablate-encoder} test whether the method is sensitive to the spatial reference and the patch representation. The window-size ablation varies the neighbourhood used to estimate the redundancy axis. Smaller windows provide a more local tissue reference, while larger windows average over more neighbours but may cross tissue boundaries. The encoder ablation compares UNI-v2, MedSigLIP-448, and an ImageNet-pretrained ViT-B/16 encoder, with Standard SA and Gated SRP evaluated within each frozen feature space.

% \paragraph{Capacity and token-role controls.}
% Tables~\ref{tab:ablate-capacity} and~\ref{tab:ablate-ln} separate the proposed mechanism from two simpler alternatives. The matched-MLP control adds comparable trainable capacity at the same insertion point but removes the spatial redundancy axis, testing whether extra parameters alone explain the improvement. The normalization ablation compares shared LayerNorm with separate CLS/patch LayerNorm, testing whether explicit token-role separation provides additional benefit beyond the projection mechanism itself.

% \paragraph{Ablation summary.}
% Together, these ablations isolate the core design choices of Gated SRP: a local spatial redundancy axis, an adaptive signed gate, identity-preserving initialization, patch-token application, and minimal added capacity. This organization distinguishes the proposed geometric correction from fixed subtraction, one-sided attenuation, generic adapter capacity, and encoder-specific effects.

==> sections/methodology-l2.tex <==
\section{Methodology}
\label{sec:methodology}
\subsection{Motivation}
\label{sec:motivation}

In computational pathology, people usually deal with whole-slide images (WSIs) and/or WSI patches, which have three key properties that constrain
attention-modification mechanisms. %
\begin{itemize}\itemsep2pt\leftmargin=1.4em
  \item \textbf{Redundancy is spatial.} Adjacent patch tokens inside tumour,
  stroma, or lymphoid regions often share cell type, staining, and
  texture, so the relevant redundancy axis is local neighbourhood
  context rather than the token's own value alone.

  \item \textbf{Projection strength is token-dependent.} A patch token inside
  homogeneous tissue may tolerate strong projection, whereas an isolated
  tumour focus may contain the slide's entire diagnostic signal.

  \item \textbf{Rare evidence may require amplification.} For isolated
  or boundary tokens, the useful signal is their disagreement with the
  neighbourhood; one-sided removal can suppress exactly that evidence.
\end{itemize}
%
XSA's three coupled choices (projection along $\hat v_i$, a fixed coefficient uniformly applied to all tokens, and one-sided removal) directly contradict the three properties above. In the next subsection, we propose the \textbf{gated spatial redundancy projection} attention, which revises the three choices accordingly.


\subsection{Gated Spatial Redundancy Projection}
\label{sec:gated-srp}
\label{sec:signed-gate}

Gated Spatial Redundancy Projection (Gated SRP) modifies only the
attention contribution $y_{i,h}$ of a visual token $i$ in head $h$.
It first defines the local common component
\begin{equation}
\label{eq:common-component}
c_{i,h} \;=\; \bigl(y_{i,h}^{\top}\hat r_{i,h}\bigr)\hat r_{i,h} = \proj_{r_{i,h}}y_{i,h},
\end{equation}
where $r_{i,h}$ is the spatial redundancy vector and $\hat r_{i,h}$ is a spatial-neighbourhood direction, as shown in Eq \ref{eq:r-def}. Then, the local common component is being multiplied by a signed, token-specific coefficient $\beta_{\mathrm{eff},\,i,h}$ (Eq~\ref{eq:beta-eff}), and subtracted from $y_{i,h}$:
\begin{equation}
\label{eq:gated-srp}
\boxed{\;\;
z_{i,h} \;=\; y_{i,h} \;-\; \beta_{\mathrm{eff},\,i,h}\,c_{i,h}
\;\;}
\qquad\text{(per head)}
\end{equation}
This single equation implements the three changes motivated above. First,
the axis $\hat r$ is spatial rather than self-referential. Second, the strength
$\beta_{\mathrm{eff}}$ varies per token and head. Lastly, the signed range
of $\beta_{\mathrm{eff}}$ lets the model choose anti-projection,
identity, projection, or reflection as local context requires.
\newline
Algorithm~\ref{alg:gated-srp} gives the per-block forward in PyTorch-style pseudocode, with each line of the highlighted block tied back to the equations defined in this section. The same forward also exposes the non-detached gate output used by the optional gate-strength regularizer.

\paragraph{Spatial redundancy axis.}
We define spatial redundancy as the local common pattern within a spatial neighbourhood. For each visual token $i$, let $\mathcal{N}(i)$ be the set of valid
spatial neighbours on the patch grid within a $n\times n$ window, where $n$ is a hyperparameter. In our experiments, we use $n=3$, which gives an 8-neighbour grid when coordinates are available, and the analogous
fixed grid for patch-level images. The head-$h$ neighbourhood mean is
\begin{equation}
\label{eq:r-def}
r_{i,h} \;=\; \frac{1}{m_i}\sum_{j\in\mathcal{N}(i)}
              \mathrm{StopGrad}(v_{j,h}),
\qquad
\hat r_{i,h} \;=\; r_{i,h}\,\big/\,\bigl(\|r_{i,h}\|_2 + \epsilon\bigr),
\qquad
m_i = |\mathcal{N}(i)|,
\end{equation}
where $\mathrm{StopGrad}(\cdot)$ denotes the stop-gradient operator and
$\epsilon$ is a small stability constant. We stop gradients through
$\hat r_{i,h}$ so that the neighbour mean is a geometric reference
rather than a trainable escape route through $W_v$. The learnable part
of the method is therefore the decision of how to use this local axis,
not the axis itself.


\begin{figure}[t]
\centering
\begin{tikzpicture}[
  >={Stealth[length=2.1mm,width=1.7mm]},
  font=\small,
  axis/.style={->, line width=0.45pt, color=gray!45},
  ref/.style={->, line width=0.95pt, color=black!85},
  xsa/.style={->, dashed, line width=0.65pt, color=gray!60},
  regarr/.style={->, line width=1.05pt},
  guide/.style={dashed, line width=0.45pt, color=gray!50},
  legenddot/.style={circle, fill, inner sep=1.45pt},
]

% ---------------------------------------------------------------------
% (a) Geometry panel. Labels live in the right legend.
% ---------------------------------------------------------------------
\begin{scope}
  \node[font=\large, anchor=west] at (-1.75,2.55) {(a)};

  % Orthogonal complement strip and axes.
  \fill[blue!6] (-0.34,-0.55) rectangle (0.34,2.28);
  \draw[axis] (-1.55,0) -- (2.35,0);
  \draw[axis] (0,-0.48) -- (0,2.43);
  \node[font=\scriptsize, color=gray!55!black, anchor=north]
    at (0,-0.58) {$\hat r^{\perp}$};

  % Main axes/vectors.
  \draw[ref] (0,0) -- (1.38,0);
  \node[font=\small, anchor=north] at (1.18,-0.05) {$\hat r$};

  \draw[xsa] (0,0) -- (0.86,0.48);
  \node[font=\scriptsize, color=gray!55!black, anchor=west]
    at (0.89,0.49) {$\hat v$ (XSA)};

  % Projection guide and shared perpendicular coordinate.
  \draw[guide] (0.92,1.62) -- (0.92,0);
  \draw[guide] (-1.08,1.62) -- (1.95,1.62);

  % Regime arrows. The legend at right names them to avoid overlap.
  \draw[regarr, color=red!65!black]       (0,0) -- (-0.92,1.62);
  \draw[regarr, color=blue!65!black]      (0,0) -- (0,1.62);
  \draw[regarr, color=black]              (0,0) -- (0.92,1.62);
  \draw[regarr, color=teal!55!black]      (0,0) -- (1.84,1.62);

  % Dots at the regime endpoints.
  \fill[red!65!black]  (-0.92,1.62) circle (1.65pt);
  \fill[blue!65!black] (0,1.62) circle (1.65pt);
  \fill[black]         (0.92,1.62) circle (1.65pt);
  \fill[teal!55!black] (1.84,1.62) circle (1.65pt);

  % Endpoint labels. The beta=0 arrow is the original y; other endpoints
  % are labelled by their signed-gate regime.
  \node[font=\scriptsize, color=red!65!black, anchor=south east]
    at (-0.95,1.70) {$z_{refl}$};
  \node[font=\scriptsize, color=blue!65!black, anchor=south east]
    at (-0.05,1.70) {$z_{proj}$};
  \node[font=\scriptsize, color=black, anchor=south west]
    at (0.5,1.70) {$z_{iden}=y$};
  \node[font=\scriptsize, color=teal!55!black, anchor=south west]
    at (1.88,1.70) {$z_{anti}$};

  % The vertical guide marks the common component (y^T r_hat) r_hat.
\end{scope}

% ---------------------------------------------------------------------
% (b) Signed range and legend panel.
% ---------------------------------------------------------------------
\begin{scope}[xshift=3.75cm, yshift=0cm]
  \node[font=\large, anchor=west] at (-0.35,2.55) {(b)};

  % Compact legend above the signed range.
  \node[font=\small\bfseries, anchor=west] at (2.35,2.25) {Signed regimes};

  \fill[red!65!black] (2.35,1.88) circle (1.7pt);
  \node[font=\scriptsize, color=red!65!black, anchor=west]
    at (2.55,1.88) {$\beta=2$: reflection};

  \fill[blue!65!black] (2.35,1.54) circle (1.7pt);
  \node[font=\scriptsize, color=blue!65!black, anchor=west]
    at (2.55,1.54) {$\beta=1$: projection};

  \fill[black] (2.35,1.20) circle (1.7pt);
  \node[font=\scriptsize, color=black, anchor=west]
    at (2.55,1.20) {$\beta=0$: identity};

  \fill[teal!55!black] (2.35,0.86) circle (1.7pt);
  \node[font=\scriptsize, color=teal!55!black, anchor=west]
    at (2.55,0.86) {$\beta<0$: anti-proj.};

  % Signed beta range inset.
  \draw[fill=blue!7, draw=blue!35!black, line width=0.35pt,
        rounded corners=1pt] (-0.15,-0.09) rectangle (2.85,0.09);
  \draw[->, line width=0.55pt] (-0.50,0) -- (3.20,0);
  \node[font=\scriptsize, anchor=west] at (3.22,0) {$\beta_{\mathrm{eff}}$};

  \foreach \x/\col/\lab in {%
      -0.15/teal!55!black/$-1$,
       0.85/black/$0$,
       1.85/blue!65!black/$1$,
       2.85/red!65!black/$2$%
  }{%
    \draw[\col, line width=0.5pt] (\x,0.12) -- (\x,-0.12);
    \fill[\col] (\x,0) circle (1.45pt);
    \node[font=\scriptsize, color=\col, anchor=north] at (\x,-0.15) {\lab};
  }

  \node[font=\scriptsize, color=blue!40!black, anchor=south]
    at (-0.15,0.13) {$-\delta$};
  \node[font=\scriptsize, color=blue!40!black, anchor=south]
    at (2.85,0.13) {$+\delta$};

  \node[font=\scriptsize, color=gray!55!black, anchor=north]
    at (1.35,-0.55)
    {$\beta_{\mathrm{eff}}=\delta\tanh(\ell_{i,h})$};
\end{scope}

\end{tikzpicture}

\caption{\textbf{Geometric regimes of the signed gate.}
\textbf{(a)} For a fixed local redundancy axis $\hat r$, changing
$\beta_{\mathrm{eff}}$ moves the output only along the $\hat r$
direction. The identity endpoint is labelled $y=z_{iden}$ here, while the
other regimes are labelled as $z$ variants: projection, reflection, and
anti-projection. The faint $\hat v$ arrow shows XSA's self-axis for
contrast.
\textbf{(b)} The signed gate places these regimes on the bounded range
$\beta_{\mathrm{eff}}=\delta\tanh(\ell_{i,h})$, with the regime selected
separately for each token and head.}
\label{fig:gated-srp-regimes}
\end{figure}



\paragraph{Signed local gate.}
The scalar $\beta_{\mathrm{eff},\,i,h}$ is produced from a gate logit
$\ell_{i,h}$ (Eq~\ref{eq:gate-logit}) by a bounded signed head:
\begin{equation}
\label{eq:beta-eff}
\beta_{\mathrm{eff},\,i,h} \;=\; \delta\cdot\tanh(\ell_{i,h})
\;\in\; (-\delta,\,+\delta).
\end{equation}
where $\delta$ is a hyperparameter controlling the range of $\beta_{\mathrm{eff},\,i,h}$. Different $\beta_{\mathrm{eff},\,i,h}$ value has different geometric meanings, as shown in Fig \ref{fig:gated-srp-regimes} and the table below:
\[
\begin{array}{c|c}
\beta_{\mathrm{eff}} & \text{operation on }c_{i,h} \\ \hline
0 & \text{identity: } z=y \\
1 & \text{projection: remove the } \hat r\text{-component} \\
2 & \text{reflection: flip the } \hat r\text{-component} \\
<0 & \text{anti-projection: amplify alignment with }\hat r .
\end{array}
\]
We use $\delta\in\{1,2\}$ as a small architectural choice: $\delta=1$
allows identity, projection, and anti-projection, while $\delta=2$ also
allows reflection. Keeping $\delta$ fixed makes this representational
choice explicit rather than hiding it inside optimization.

\paragraph{Factored gate logit.}
The logit combines token-level context with head-level alignment:
\begin{equation}
\label{eq:gate-logit}
\ell_{i,h} \;=\;
  \underbrace{g_{\text{tok}}(d^{\text{tok}}_i)}_{\text{shared across heads}}
  \;+\;
  \underbrace{w_h^{\top}d^{\text{head}}_{i,h} + b_h}_{\text{head-specific}}
  \;+\;
  \underbrace{b_{l,h}}_{\text{per-(layer, head) bias}}\,,
\end{equation}
where $g_{\text{tok}}$ is a two-layer MLP with GELU activation, and $d^{\text{tok}}_i\in\mathbb{R}^{T_t}$ and $d^{\text{head}}_{i,h}\in\mathbb{R}^{T_h}$ are the token/head-level diagnostics vectors. The diagnostic vectors are defined as
\newline
\begin{equation}
\label{eq:diag-tok}
d^{\text{tok}}_i \;=\; \bigl[\,
  h_{\text{local},\,i},\;\;
  m_i/8,\;\;
  \log(1+m_i)
\,\bigr],
\end{equation}
\begin{equation}
\label{eq:diag-head}
d^{\text{head}}_{i,h} \;=\; \bigl[\,
  \cos(y_{i,h},\hat r_{i,h}),\;\;
  |\cos(y_{i,h},\hat r_{i,h})|,\;\;
  \log(1+\|y_{i,h}\|_2)
\,\bigr],
\end{equation}
with $T_t=T_h=3$ in the default gate. The token features summarise
whether the local tissue context is reliable enough to project
against:
\begin{itemize}\itemsep1pt\leftmargin=1.4em
  \item $h_{\text{local},\,i}=m_i^{-1}\sum_{j\in\mathcal{N}(i)}
        \cos(\phi_i,\phi_j)$ is the mean cosine similarity between the
        raw patch embedding $\phi_i$ and its neighbours, so it
        measures how homogeneous the surrounding tissue actually is.
  \item $m_i/8$ is the linear fraction of valid neighbours, marking
        boundary and corner tokens whose spatial context is
        incomplete.
  \item $\log(1+m_i)$ is a log-confidence proxy for $\hat r_{i,h}$:
        the variance of the neighbour mean scales as $1/m_i$, so this
        term lets the gate shrink $\beta_{\rm eff}$ when the axis is
        built from few samples.
\end{itemize}
The head features describe how the current attention contribution
$y_{i,h}$ relates to that axis:
\begin{itemize}\itemsep1pt\leftmargin=1.4em
  \item $\cos(y_{i,h},\hat r_{i,h})$ is the signed alignment of the
        head output with the redundancy axis, indicating whether
        subtracting $c_{i,h}$ acts as projection or anti-projection.
  \item $|\cos(y_{i,h},\hat r_{i,h})|$ is the unsigned alignment
        magnitude, separating how much of $y_{i,h}$ lies along
        $\hat r_{i,h}$ from in which direction.
  \item $\log(1+\|y_{i,h}\|_2)$ is the log-magnitude of the
        contribution being projected, so the gate can avoid
        corrections on tokens whose attention output is essentially
        zero.
\end{itemize}

% Here
% $h_{\text{local},\,i} =
%  m_i^{-1}\sum_{j\in\mathcal{N}(i)}\cos(\phi_i,\phi_j)$
% is the mean cosine similarity between the raw patch embedding
% $\phi_i$ and its neighbours. Thus $d^{\text{tok}}$ encodes how
% homogeneous and well-supported the local tissue context is, while
% $d^{\text{head}}$ encodes whether the current head output actually
% lies along that context direction.

The factorization of the gate logit is intentional: the shared token term decides whether
the local tissue context is redundant; the per-head term decides how
strongly this head's attention output aligns with that context, and
$b_{l,h}$ absorbs layer/head-specific scale shifts. This keeps the
gate interpretable and small, with
$\mathcal{O}(T_t h_{\text{mlp}} + H T_h)$ parameters per active block.

% \begin{figure}[t]
% \begin{lstlisting}[style=gsrpcode,
%   caption={Gated SRP attention block in PyTorch-style pseudocode.
%   Standard multi-head self-attention (lines~1--4) is unchanged from a
%   reference implementation; the tinted block (lines~5--21) contains
%   the Gated-SRP additions, mapped one-to-one to the equations of
%   \S\ref{sec:gated-srp}. Tensor shapes use $B$ batch, $H$ heads, $N$
%   tokens, $d$ head-dim. \texttt{nbr\_idx} and \texttt{nbr\_mask} carry
%   the per-token 8-neighbour graph; \texttt{h\_local} is the
%   precomputed local-homogeneity score from
%   Eq.~\eqref{eq:diag-tok}; \texttt{eps} is the stability constant of
%   Eq.~\eqref{eq:r-def}; \texttt{delta}~$\in\{1, 2\}$ sets the signed
%   range of Eq.~\eqref{eq:beta-eff}.},]
% # Standard multi-head self-attention
% Q, K, V = split_heads(x @ Wq, x @ Wk, x @ Wv)
% A = softmax(Q @ K.transpose(-2,-1) / sqrt(d))
% Y = A @ V                                # SA output

% # === Gated SRP ============================
% r = gather(V.detach(), nbr_idx).mean(-2)   # Eq. 4
% r_hat = r / (r.norm(-1, keepdim=True) + eps)
% c = (Y * r_hat).sum(-1, keepdim=True) * r_hat

% m = nbr_mask.sum(-1).float()
% d_tok = stack([h_local, m/8, log1p(m)], -1).detach()
% cos_yr = (Y * r_hat).sum(-1)
% d_head = stack([cos_yr, cos_yr.abs(),
%                 log1p(Y.norm(-1))], -1).detach()

% logit = (g_tok(d_tok)[:,None,:,None]
%          + einsum("bhnt,ht->bhn", d_head, w_h)[...,None]
%          + b_h.view(1,H,1,1)
%          + b_lh.view(1,H,1,1))
% beta = delta * tanh(logit)                 # Eq. 7
% Z = Y - beta * c                           # replaces Y, Eq. 1
% # === end Gated SRP ========================

% out = x + Wo @ merge_heads(Z)              # residual + output projection
% \end{lstlisting}
% \end{figure}

\begin{algorithm}[t]
\caption{Gated SRP attention block in PyTorch-style pseudocode.
% The Gated-SRP additions (lines~4--12)
% realize Eqs.~\eqref{eq:r-def}--\eqref{eq:gated-srp}. Tensor shapes
% use $B$ batch, $H$ heads, $N$ tokens, $d$ head-dim.
% \texttt{nbr\_idx}/\texttt{nbr\_mask} carry the per-token 8-neighbour
% graph; \texttt{h\_local} is the precomputed local-homogeneity score;
% \texttt{eps} is the stability constant; \texttt{delta}~$\in\{1, 2\}$
% sets the signed range of Eq.~\eqref{eq:beta-eff}.}
}
\label{alg:gated-srp}
\footnotesize
\begin{algorithmic}[1]
\Require \texttt{x}; projections \texttt{Wq, Wk, Wv, Wo}; neighbour
  graph \texttt{nbr\_idx, nbr\_mask}; \texttt{h\_local}; gate
  parameters \texttt{g\_tok, w\_h, b\_h, b\_lh}; range \texttt{delta}.
\Ensure \texttt{out} (replaces the standard attention-block output).
\Statex \textbf{\textit{\# Standard multi-head self-attention}}
\State \texttt{Q, K, V = split\_heads(x @ Wq, x @ Wk, x @ Wv)}
\State \texttt{A = softmax(Q @ K.transpose(-2,-1) / sqrt(d))}
\State \texttt{Y = A @ V} \Comment{SA output}
\Statex \textbf{\textit{\# === Gated SRP ===}}
\State \texttt{r = gather(V.detach(), nbr\_idx).mean(-2)}
  \Comment{Eq.~\eqref{eq:r-def}}
\State \texttt{r\_hat = r / (r.norm(-1, keepdim=True) + eps)}
\State \texttt{c = (Y * r\_hat).sum(-1, keepdim=True) * r\_hat}
  \Comment{Eq.~\eqref{eq:common-component}}
\State \texttt{m = nbr\_mask.sum(-1).float()}
\State \texttt{d\_tok = stack([h\_local, m/8, log1p(m)], -1).detach()}
  \Comment{Eq.~\eqref{eq:diag-tok}}
\State \texttt{y\_norm = Y.norm(-1)}
\State \texttt{cos\_yr = (Y * r\_hat).sum(-1) / (y\_norm + eps)}
\State \texttt{d\_head = stack([cos\_yr, cos\_yr.abs(),}
\Statex \hspace{3.2em}\texttt{log1p(y\_norm)], -1).detach()}
  \Comment{Eq.~\eqref{eq:diag-head}}
\State \texttt{logit = g\_tok(d\_tok)[:,None,:,None]}
\Statex \hspace{3.2em}\texttt{+ einsum("bhnt,ht->bhn", d\_head, w\_h)[...,None]}
\Statex \hspace{3.2em}\texttt{+ b\_h.view(1,H,1,1) + b\_lh.view(1,H,1,1)}
  \Comment{Eq.~\eqref{eq:gate-logit}}
\State \texttt{beta = delta * tanh(logit)}
  \Comment{Eq.~\eqref{eq:beta-eff}}
% \State \texttt{cache\_for\_loss(beta)}
%   \Comment{active signed-gate blocks only; optional regularization}
\State \texttt{Z = Y - beta * c}
  \Comment{replaces \texttt{Y}; Eq.~\eqref{eq:gated-srp}}
\Statex \textbf{\textit{\# === end Gated SRP ===}}
\State \texttt{out = x + Wo @ merge\_heads(Z)}
  \Comment{standard residual + output projection}
\end{algorithmic}
\end{algorithm}

\paragraph{Identity initialization.}
The output layer of $g_{\text{tok}}$, all per-head weights
$\{w_h,b_h\}$, and all layer/head biases $b_{l,h}$ are initialized to
zero. The hidden layer of $g_{\text{tok}}$ keeps its standard
initialization. Consequently $\ell_{i,h}=0$ and
$\beta_{\mathrm{eff},\,i,h}=0$ for every token and head at step~1, so
Eq.~\eqref{eq:gated-srp} exactly recovers standard self-attention.
Any non-zero projection is therefore learned during optimization rather
than injected by the architecture at initialization.

\paragraph{Default gradient convention.}
Both diagnostic vectors $d^{\text{tok}}_i$ and $d^{\text{head}}_{i,h}$ are detached before being passed to the gate.
Thus, gate parameters are trained through their effect on
$z_{i,h}$, but the upstream attention projection does not receive an
additional gradient path through feature construction. When the
gate-strength regularizer is enabled, it uses a non-detached cache of $\beta_{\mathrm{eff}}$ itself,
so its gradients still flow into the gate parameters; only the
diagnostic-feature construction remains stop-gradient. This separates
the specified mechanism from the ``live-input'' ablation used in our
experiments, where gradients through the diagnostic features are
allowed and analyzed separately.

\paragraph{Application scope.}
Gated SRP is applied only to visual patch tokens; the
\textsc{cls} token is left unchanged. When the classifier reads only
\textsc{cls}, patch-token projection in the final attention block has
no same-block path to the loss, so we omit the gate in that final
block. The gate-regularization set is the same set of active signed-gate
blocks; the final dead-path block contributes neither parameters nor a
regularization term. The modified heads are concatenated and passed through the
standard output projection and residual connection exactly as in the
baseline transformer.

\paragraph{Implementation summary.}
Each active block adds three lightweight pieces: a spatial neighbour
gather over $V$, the token MLP $g_{\text{tok}}$, and a per-head linear
gate. In our settings, this contributes less than $0.02\%$ of the
trainable parameter budget. The method is therefore primarily an
inductive-bias change rather than a substantial capacity increase. The
optional regularizer reuses the already-computed $\beta_{\mathrm{eff}}$
cache and adds no additional forward computation. The full per-block
implementation fits in roughly twenty lines (Algorithm~\ref{alg:gated-srp}).


\paragraph{Training objective.}
For every task, we train with the generic objective $\mathcal{L}=\mathcal{L}_{\mathrm{task}}+\mathcal{L}_{\mathrm{reg}}$, where $\mathcal{L}_{\mathrm{task}}$ is the task's native loss and the regularization term is added independently of that loss form. For Gated SRP, $\mathcal{L}_{\mathrm{reg}}=\lambda_{\mathrm{gate}}|\mathcal{A}|^{-1}\sum_{a\in\mathcal{A}}\operatorname*{mean}_{b,h,i}\bigl[(\beta_{\mathrm{eff},\,b,i,h}^{(a)})^2\bigr]$, averaged over active signed-gate blocks and real visual tokens. This term acts as a safety lock. Since $\beta_{\mathrm{eff}}=0$ recovers standard self-attention, the gate is penalized for moving away from the SA baseline unless non-zero gating improves the task loss enough to justify the change, so an unhelpful gate is driven toward the no-op SA solution rather than a harmful projection.



% \begin{algorithm}[t]
% \caption{Gated SRP — one attention block.
% \textsc{cls} bypasses unmodified; the final attention block omits the
% gate (Application scope, \S\ref{sec:gated-srp}). Each line below is
% applied per visual patch token $i$ and head $h$.}
% \label{alg:gated-srp}
% \begin{algorithmic}[1]
% \Require Per-head SA outputs $y_{i,h}$ (Eq.~\ref{eq:sa-weights});
%   value vectors $v_{j,h}$; neighbour graph $\mathcal{N}$ with
%   $m_i = |\mathcal{N}(i)|$; raw patch embeddings $\phi$; gate
%   parameters $\bigl\{g_{\text{tok}},\, w_h,\, b_h,\, b_{l,h}\bigr\}$;
%   range $\delta \in \{1, 2\}$.
% \Ensure Modified contributions $z_{i,h}$ that replace $y_{i,h}$ before
%   the output projection and residual.
% \Statex
% \State $r_{i,h} \;\gets\; m_i^{-1}\sum_{j \in \mathcal{N}(i)}
%         \mathrm{sg}\bigl(v_{j,h}\bigr)$
% \Comment{neighbour mean of values, Eq.~\ref{eq:r-def}}

% \State $\hat r_{i,h} \;\gets\; r_{i,h}\,/\,(\|r_{i,h}\|_2 + \epsilon)$
% \Comment{unit redundancy axis}

% \State $c_{i,h} \;\gets\; \bigl(y_{i,h}^{\top}\hat r_{i,h}\bigr)\,
%         \hat r_{i,h}$
% \Comment{common component, Eq.~\ref{eq:common-component}}

% \State $d^{\text{tok}}_i \;\gets\; \mathrm{sg}\!\bigl(
%         \bigl[\,h_{\text{local},\,i},\;\; m_i/8,\;\; \log(1{+}m_i)\,\bigr]
%         \bigr)$
% \Comment{per-token diagnostics, Eq.~\ref{eq:diag-tok}}

% \State $d^{\text{head}}_{i,h} \;\gets\; \mathrm{sg}\!\bigl(
%         \bigl[\,\cos(y_{i,h},\hat r_{i,h}),\;\;
%                 |\cos(y_{i,h},\hat r_{i,h})|,\;\;
%                 \log(1{+}\|y_{i,h}\|_2)\,\bigr]
%         \bigr)$
% \Comment{per-head diagnostics, Eq.~\ref{eq:diag-head}}

% \State $\ell_{i,h} \;\gets\; g_{\text{tok}}(d^{\text{tok}}_i)
%         \;+\; w_h^{\top} d^{\text{head}}_{i,h} \;+\; b_h
%         \;+\; b_{l,h}$
% \Comment{factored gate logit, Eq.~\ref{eq:gate-logit}}

% \State $\beta_{\mathrm{eff},\,i,h} \;\gets\;
%         \delta \cdot \tanh(\ell_{i,h}) \;\in\; (-\delta,\,+\delta)$
% \Comment{signed bounded coefficient, Eq.~\ref{eq:beta-eff}}

% \State $z_{i,h} \;\gets\; y_{i,h} \;-\; \beta_{\mathrm{eff},\,i,h}
%         \, c_{i,h}$
% \Comment{Eq.~\ref{eq:gated-srp}; identity at step~1 since
%          $\beta_{\mathrm{eff}}\!=\!0$ at zero-init}
% \end{algorithmic}
% \end{algorithm}

% \subsection{Gated Spatial Redundancy Projection (GSRP)}
% \label{sec:gated-srp}

% We replace XSA's projection rule with a single composite operation with two core designs
% that addresses motivations~(i)–(iii) of \S\ref{sec:motivation} jointly:
% \begin{equation}
% \label{eq:gated-srp}
% \boxed{\;\;
% z_{i,h} \;=\; y_{i,h} \;-\; \beta_{\text{eff},\,i,h}\,
%             \bigl(\,y_{i,h}^{\top}\hat r_{i,h}\,\bigr)\,\hat r_{i,h}
% \;\;}
% \qquad\text{(per head)}
% \end{equation}
% where \textbf{(a)}~$\hat r_{i,h}$ is a unit vector along the local neighbourhood mean of value vectors, representing the local redundancy axis; and
% \textbf{(b)}~$\beta_{\text{eff},\,i,h}\!\in\!\mathbb{R}$ is a learned adaptive
% per-(token, head) coefficient produced by a small gate network, constrained to a signed bounded range. The remainder of this subsection defines each
% component, with the rationale for every design choice tied back to
% the motivation it implements.



% \paragraph{Local redundancy axis}
% For each token $i$, let $\mathcal{N}(i)$ denote its set of nearest
% spatial neighbours within a window on the slide grid. We use a $3\times3$ window in all our experiments where $|\mathcal{N}(i)|=8$. The head-$h$ neighbourhood mean and its unit
% vector are
% \begin{equation}
% \label{eq:r-def}
% r_{i,h} \;=\; \frac{1}{|\mathcal{N}(i)|}\sum_{j\in\mathcal{N}(i)}
%               \mathrm{sg}(v_{j,h}),
% \qquad
% \hat r_{i,h} \;=\; r_{i,h}\,\big/\,\bigl(\|r_{i,h}\|_2 + \epsilon\bigr),
% \end{equation}
% where $\mathrm{sg}(\cdot)$ denotes the stop-gradient operator and
% $\epsilon$ is a small constant for numerical stability. Stop-gradient
% is applied to $\hat r_{i,h}$ because we want to treat it as a
% (slowly-varying) geometric reference rather than a learned parameter
% — the only effect of Eq.~\eqref{eq:gated-srp} on the loss is then
% mediated by $\beta_{\text{eff}}$, the single learnable scalar per
% (token, head). Without the stop-gradient, gradients would flow back
% through the neighbour graph into $W_v$, turning the projection into a
% de-facto free-form linear transformation and entangling the value
% projection with the GSRP correction.

% \paragraph{Local adaptive projection coefficient.}
% The coefficient $\beta_{\text{eff},\,i,h}$ in Eq.~\eqref{eq:gated-srp}
% is produced by passing a scalar gate logit $\ell_{i,h}$ through a
% $\tanh$ head with explicit range bound $\delta>0$:
% \begin{equation}
% \label{eq:beta-eff}
% \beta_{\text{eff},\,i,h} \;=\; \delta\cdot\tanh(\ell_{i,h})
% \;\in\; (-\delta,\,+\delta).
% \end{equation}
% Eq.~\eqref{eq:beta-eff} together with Eq.~\eqref{eq:gated-srp}
% exposes four geometric regimes on a single one-dimensional knob:
% $\beta_{\text{eff}}\!=\!0$ leaves $z_{i,h}\!=\!y_{i,h}$
% (\emph{identity}); $\beta_{\text{eff}}\!=\!1$ removes the component
% of $y$ along $\hat r$ (orthogonal-complement \emph{projection});
% $\beta_{\text{eff}}\!=\!2$ flips that component (\emph{reflection}
% through the orthogonal hyperplane); and $\beta_{\text{eff}}\!<\!0$
% amplifies the alignment with $\hat r$ (\emph{anti-projection}, the
% rare-cell regime that motivation~(iii) demands). Choosing
% $\delta\!=\!1$ yields the bounded interval $(-1, +1)$, which contains
% identity, projection, and anti-projection but excludes reflection;
% $\delta\!=\!2$ contains all four regimes. We treat $\delta$ as a
% small architectural hyperparameter rather than a learnable variable,
% because its value materially changes which geometric regimes the gate
% can \emph{represent}, and a learned $\delta$ would collapse this
% representational choice to whichever value happens to minimise the
% training objective along a particular optimisation trajectory.

% The logit $\ell_{i,h}$ is itself produced by a deliberately
% \emph{factored} composition of inputs from two sources: a vector of
% \emph{per-token diagnostics}
% $d^{\text{tok}}_i\!\in\!\mathbb{R}^{T_t}$ (shared across heads) that
% summarises the redundancy of the token's local neighbourhood, and a
% vector of \emph{per-head diagnostics}
% $d^{\text{head}}_{i,h}\!\in\!\mathbb{R}^{T_h}$ that summarises the
% head-specific alignment of $y_{i,h}$ with $\hat r_{i,h}$. The two
% combine through
% \begin{equation}
% \label{eq:gate-logit}
% \ell_{i,h} \;=\;
%   \underbrace{\mathrm{MLP}_{\text{tok}}(d^{\text{tok}}_i)}_{\text{shared across heads}}
%   \;+\;
%   \underbrace{w_h^{\top}d^{\text{head}}_{i,h} + b_h^{\text{head}}}_{\text{per-head linear}}
%   \;+\;
%   \underbrace{b_{l,h}}_{\text{per-(layer, head) bias}}\,,
% \end{equation}
% where $\mathrm{MLP}_{\text{tok}}\!:\!\mathbb{R}^{T_t}\!\to\!\mathbb{R}$
% is a 2-layer MLP with hidden size $h_{\text{mlp}}\!\in\!\{16,32,64\}$
% and GELU activation, and $\{w_h, b_h^{\text{head}}, b_{l,h}\}_{h=1}^H$
% are per-head parameters owned by this layer's gate. The factorisation
% mirrors the empirical structure of the decision to be made: the bulk
% of ``how much projection should this token absorb'' is a function of
% \emph{local context} (homogeneity, neighbour count) which is identical
% across the heads of a token; the per-head linear correction
% accommodates head specialisation (different heads read different
% sub-aspects of $y$); and the per-(layer, head) bias accommodates
% layer-specific drift in the magnitude of $y$ as depth grows. A
% monolithic per-(token, head) MLP would burn $H\!\cdot\!T_h$
% parameters per layer on information already captured by the shared
% token MLP; the factored form has
% $\mathcal{O}(H\,T_h + T_t\,h_{\text{mlp}})$ gate parameters per layer,
% which for our settings is below $0.02\%$ of the model's trainable
% parameter budget.

% The two diagnostic vectors are concretely defined as
% \begin{equation}
% \label{eq:diag-tok}
% d^{\text{tok}}_i \;=\; \bigl[\,
%   h_{\text{local},\,i},\;\;
%   |\mathcal{N}(i)|/8,\;\;
%   \log(1+|\mathcal{N}(i)|)
% \,\bigr],
% \end{equation}
% \begin{equation}
% \label{eq:diag-head}
% d^{\text{head}}_{i,h} \;=\; \bigl[\,
%   \cos(y_{i,h},\hat r_{i,h}),\;\;
%   |\cos(y_{i,h},\hat r_{i,h})|,\;\;
%   \log(1+\|y_{i,h}\|_2)
% \,\bigr],
% \end{equation}
% with $T_t = T_h = 3$ in our experiments. The components of
% $d^{\text{tok}}_i$ encode redundancy-density signals that are
% available before the attention output is computed. The first is the
% \emph{local-homogeneity score}
% $h_{\text{local},\,i} =
%  \tfrac{1}{|\mathcal{N}(i)|}\!\sum_{j\in\mathcal{N}(i)}\!\cos(\phi_i,\phi_j)$,
% the mean cosine similarity between patch $i$'s raw embedding $\phi_i$
% and those of its 8 spatial neighbours, computed once during
% preprocessing; a high $h_{\text{local}}$ flags that the token sits
% inside a uniform tissue region and is a strong candidate for
% projection. The second is the \emph{normalised neighbour count}
% $|\mathcal{N}(i)|/8$, which equals $1$ for interior tokens and is
% lower for edge tokens with fewer than 8 valid spatial neighbours.
% The third is the \emph{log-scaled neighbour count}
% $\log(1+|\mathcal{N}(i)|)$, which gives the gate a smoother handle
% on the count scale than the raw value. Together these three
% components carry the redundancy-density signal that motivation~(ii)
% asks for: dense homogeneous neighbourhoods drive the gate logit
% upward and the token absorbs more projection, while sparse or
% heterogeneous neighbourhoods suppress the logit so the projection
% is held back.

% The components of $d^{\text{head}}_{i,h}$ encode post-attention
% alignment signals computed from $y_{i,h}$ and $\hat r_{i,h}$. The
% first is the \emph{signed cosine} $\cos(y_{i,h}, \hat r_{i,h})$,
% which is positive when the attention output already moves along the
% redundancy axis (a signal that projection will remove a real
% component of $y_{i,h}$) and negative when it moves against it (a
% signal that the rare-cell anti-projection regime of motivation~(iii)
% may apply). The second is the \emph{unsigned alignment magnitude}
% $|\cos(y_{i,h}, \hat r_{i,h})|$, which gives the gate a sign-agnostic
% measure of how strongly $y_{i,h}$ is oriented along $\hat r_{i,h}$.
% The third is the \emph{log-scaled output magnitude}
% $\log(1+\|y_{i,h}\|_2)$, which prevents the gate from being dominated
% by outlier-magnitude tokens.

% Finally, the gate is \emph{identity-initialised}: the output-path
% parameters of $\mathrm{MLP}_{\text{tok}}$ (output-layer weight and
% bias) along with all per-head parameters
% $\{w_h, b_h^{\text{head}}, b_{l,h}\}$ are set to zero at construction.
% Hidden-layer weights of $\mathrm{MLP}_{\text{tok}}$ keep their default
% Kaiming initialisation, so non-zero gradients flow into the gate as
% soon as the output layer leaves zero. With this choice
% $\ell_{i,h}\!=\!0$ at training step~1 across every token, head, layer,
% and example, hence $\beta_{\text{eff},\,i,h}\!=\!\delta\tanh(0)\!=\!0$,
% hence $z_{i,h}\!=\!y_{i,h}$ exactly. Combined with the standard
% residual at the block boundary, the entire transformer recovers its
% un-modified forward pass at step~1, so any subsequent effect of the
% gate emerges through optimisation rather than through an architectural
% prior at initialisation. This avoids the failure mode in which a
% freshly-introduced module hurts the model before its parameters have
% learned anything useful, and lets us interpret any post-training
% effect of the gate as a genuine optimisation signal.

% \paragraph{Detached gate inputs.}
% By default both diagnostic vectors $d^{\text{tok}}_i$ and
% $d^{\text{head}}_{i,h}$ are stop-gradient. The gate's parameters
% therefore receive gradient signal only through the projection in
% Eq.~\eqref{eq:gated-srp}; the upstream attention parameters
% $W_q, W_k, W_v$ do not see a gradient path through the diagnostic
% features. \emph{Rationale:} this keeps the gate's only mechanism for
% shaping training the geometric projection it is supposed to control.
% We do study an alternative ``live-input'' regime that lets the
% head-feature gradient flow back into $y$ in
% \S\ref{sec:exp-detach}; it produces small but architecture-specific
% side effects whose mechanism we attribute to a side-channel gradient
% through the magnitude of $y$, and which our experiments treat as a
% separate ablation rather than the default specification.

% \paragraph{Putting the operation together.}
% A single Gated-SRP block performs the following sequence: standard
% self-attention (Eq.~\ref{eq:sa-weights}) produces $y_{i,h}$;
% neighbour-gather + mean (Eq.~\ref{eq:r-def}) produces the unit
% redundancy axis $\hat r_{i,h}$ from a stop-gradient copy of
% $\{v_{j,h}\}$; the diagnostic vectors
% (Eqs.~\ref{eq:diag-tok}--\ref{eq:diag-head}) are computed and
% detached; the factored gate (Eq.~\ref{eq:gate-logit}) and the
% $\delta\tanh$ head (Eq.~\ref{eq:beta-eff}) produce
% $\beta_{\text{eff},\,i,h}$; and the projection
% (Eq.~\ref{eq:gated-srp}) yields $z_{i,h}$, which then enters the
% standard residual addition unchanged. The entire mechanism adds three
% small modules per attention block — an 8-NN gather of $v$, a
% two-layer token MLP, and a per-head linear — and at our settings
% contributes $<\!0.02\%$ to the model's trainable parameter budget.

